MimIR: An Extensible and Type-Safe Intermediate Representation for the DSL Age

Traditional compilers, designed for optimizing low-level code, fall short when dealing with modern, computation-heavy applications like image processing, machine learning, or numerical simulations. Optimizations should understand the primitive operations of the specific application domain and thus happen on that level. Domain-specific languages (DSLs) fulfill these requirements. However, DSL compilers reinvent the wheel over and over again as standard optimizations, code generators, and general infrastructure & boilerplate code must be reimplemented for each DSL compiler. This paper presents MimIR, an extensible, higher-order intermediate representation. At its core, MimIR is a pure type system and, hence, a form of a typed lambda calculus. Developers can declare the signatures of new (domain-specific) operations, called "axioms". An axiom can be the declaration of a function, a type constructor, or any other entity with a possibly polymorphic, polytypic, and/or dependent type. This way, developers can extend MimIR at any low or high level and bundle them in a "plugin". Plugins extend the compiler and take care of optimizing and lowering the plugins' axioms. We show the expressiveness and effectiveness of MimIR in three case studies: Low-level plugins that operate at the same level of abstraction as LLVM, a regular-expression matching plugin, and plugins for linear algebra and automatic differentiation. We show that in all three studies, MimIR produces code that has state-of-the-art performance.

==> fig/compile.tex <==
%\begin{figure}[t]
    %\begin{subcaptionblock}{\textwidth}
        \begin{lstlisting}[float=t,caption=The \texttt{\%compile} plugin to declare and compose optimizations (excerpt).,label=lst:compile]
            axm %compile.Phase: *;
            axm %compile.Pass:  *;
            .Pi %compile.Pipeline  = PI %compile.Phase -> %compile.Pipeline;
            .Pi %compile.PassList  = PI %compile.Pass  -> %compile.PassList;
            axm %compile.pipe:       %compile.Pipeline;
            axm %compile.pass_list:  %compile.PassList;
            axm %compile.pass_phase: %compile.PassList -> %compile.Phase;
        \end{lstlisting}
        %\vspace{-1.ex}
        %\caption{
        %\label{lst:compile}
        %\vspace{1.ex}
    %\end{subcaptionblock}
    %\begin{subcaptionblock}{\textwidth}
    %    \begin{lstlisting}
    %        lam default_compile(): %compile.Pipeline =
    %          %compile.pipe
    %            // ...
    %            (%compile.single_pass_phase %compile.eta_red_pass)
    %            (%compile.single_pass_phase (plugin_cond_pass (%compile.matrix_plugin, matrix_lower_phase)))
    %            // ...
    %    \end{lstlisting}
    %    \vspace{-1.ex}
    %    \caption{The \texttt{\%opt} plugin.}
    %    \label{lst:opt}
    %    \vspace{-1.ex}
    %\end{subcaptionblock}
    %\caption{\mimir's modular and extensible compilation infrastructure (excerpt).}
    %\label{lst:compile_opt}
%\end{figure}


==> fig/fun.tex <==
\begin{figure}[t]
    \centering
    \begin{subcaptionblock}{.55\textwidth}
        \begin{lstlisting}[basicstyle=\ttfamily\tiny,xleftmargin=1ex,xrightmargin=1ex]
            let f = LAM   (T: *)((x y: T), return: T -> BOT): BOT = return x;
            let f = cn (T: *)((x y: T), return: Cn T)    = return x;
            let f = fn (T: *) (x y: T): T                 = return x;
        \end{lstlisting}
        \vspace{-1.ex}
        \caption{Curried functions \& continuations}
        \label{lst:fun_expr}
    \end{subcaptionblock}%
    \begin{subcaptionblock}{.17\textwidth}
        \begin{lstlisting}[basicstyle=\ttfamily\tiny,xleftmargin=1ex,xrightmargin=1ex]
            lam f/*...*/;
            con f/*...*/;
            fun f/*...*/;
        \end{lstlisting}
        \vspace{-1.ex}
        \caption{Named}
        \label{lst:fun_decl}
    \end{subcaptionblock}%
    \begin{subcaptionblock}{.27\textwidth}
        \begin{lstlisting}[basicstyle=\ttfamily\tiny,xleftmargin=1ex,xrightmargin=1ex]
            PI  [T: *][[T, T], T -> BOT] -> BOT
            Cn[T: *][[T, T], Cn T]
            Fn[T: *] [T, T] -> T
        \end{lstlisting}
        \vspace{-1.ex}
        \caption{Curried function types}
        \label{lst:fun_type}
    \end{subcaptionblock}
    \\[1ex]
    \begin{subcaptionblock}{\textwidth}
        \begin{lstlisting}[basicstyle=\ttfamily\tiny,xleftmargin=1ex,xrightmargin=1ex]
            let f = LAM(T: *)@tt: (PI_: [[T, T], PI_: T -> BOT] -> BOT) = LAM(xyr: [[T, T], PI_: T -> BOT])@ff: BOT = xyr#1_2 xyr#0_2#0_2;
        \end{lstlisting}
        \vspace{-1.ex}
        \caption{Desugared version of \lstinline|f|}
        \label{lst:fun_desugared}
    \end{subcaptionblock}
    \caption{
        Syntactic sugar for patterns, curried functions, and function types.
        All definitions of \lstinline|f| are equivalent;
        \lstinline|f|'s type can be expressed by any expression in \ref{lst:fun_type}.
        These are equivalent, too.}
    \label{lst:sugar}
\end{figure}


==> fig/grammar.tex <==
\begin{figure}
    \begin{footnotesize}
    \begin{equation*}
        \begin{array}{rcll}
            \hul{e},\hul{T},\hul{U},\hul{s} & \Coloneqq & \hlstar \mid \hlsquare \mid \hl{$\bot$} \mid \key{Nat} \mid \hl{\key{Idx}} \mid \hl{n} \mid \hl{i$_\texttt{n}$} & \textit{Star / Box / Bottom / Nat / Idx / Literal} \quad \hl{i},\hl{n} \in \mathbb{N} \quad \hl{i} < \hl{n} \\
                                            & \mid      & \hl{x} \mid \hl{\key{let} x = \ul{e}\lstinline|;|\ \ul{e}} \mid \hl{\key{axm} x:\ul{T}; \ul{e}}                        & \textit{Var / Let / Axiom}  \\
                                            & \mid      & \hl{$\Pi$ x:\ul{T} $\to$ \ul{U}} \mid \hl{$\lambda$ x:\ul{T}@\hl{e}:\ul{U} = \ul{e}} \mid \hl{\ul{e}\ \ul{e}}     & \textit{Pi / Lam / App}             \\
                                            & \mid      & \hl{[}\overline{\hl{x:\ul{T}}}\hl{]} \mid \hl{(}\overline{\hul{e}}\hl{)} \mid \hl{\arr{x:\ul{e}; \ul{T}}} \mid \hl{\pack{x:\ul{e}; \ul{e}}} \mid \hl{\ul{e}\#\ul{e}}   & \textit{Sigma / Tuple / Array / Pack / Extract}            \\
        \end{array}
    \end{equation*}
    \end{footnotesize}
    \caption{\mimir's Syntax}
    \label{fig:syntax}
\end{figure}
%\begin{figure}
    %\begin{footnotesize}
    %\begin{align*}
        %a &= b
        %%\hl{\ul{T} $\to$ \ul{U}}                   &= \hl{$\Pi$ \textunderscore:\ul{T} $\to$ \ul{U}} \\
        %%\hl{\key{lam} x_f x:\ul{T}@\hl{e}:\ul{U}  &= \hl{$\lambda$ x:\ul{T}@(\hl{e}):\ul{U}  &= \ul{e}}
    %\end{align*}
    %\end{footnotesize}
%\end{figure}


==> fig/loop.tex <==
\begin{wrapfigure}{r}{.3\textwidth}
    \centering
    \vspace{-2.9ex}
    \begin{subcaptionblock}{\linewidth}
        \begin{lstlisting}[language=Rust]
            let mut x = 1;// stack alloc
            let     z = read();
            let mut y = z;// stack alloc
            while (dontknow()) {
                if y != z { x = 2; }
                x = 2 - x;
                if x != 1 { y = 2; }
            }
            foo(x);
        \end{lstlisting}
        \vspace{-1ex}
        \caption{Unoptimized}\label{fig:mutual_opt:unopt}
        \vspace{1ex}
    \end{subcaptionblock}
    \begin{subcaptionblock}{\linewidth}
        \begin{lstlisting}[language=Rust]]
            read();
            while (dontknow()) {}
            foo(1);
        \end{lstlisting}
        \vspace{-1ex}
        \caption{Optimized}\label{fig:mutual_opt:opt}
        \vspace{1ex}
    \end{subcaptionblock}
    \vspace{-6ex}
    \caption{Optimizer in action.}
    \vspace{-1ex}
    \label{fig:mutual_opt}
\end{wrapfigure}


==> fig/map_reduce.tex <==
\begin{wraptable}{r}{.38\textwidth}
    \centering
    \vspace{-2.9ex}
    \begin{footnotesize}
        \begin{tabular}{lrcl}
            \toprule
            Operation & \multicolumn{3}{c}{\texttt{mapReduce} call} \\
            \midrule
            matrix-matrix product       & $ij$  & $\mathclap{\gets_+}$ & $ik \cdot kj$ \\
            summation of all entries    &       & $\mathclap{\gets_+}$ & $ij$          \\
            transpose                   & $ij$  & $\mathclap{\gets_+}$ & $ji$          \\
            column-wise summation       & $ij$  & $\mathclap{\gets_+}$ & $j$           \\
            matrix-vector product       & $ij$  & $\mathclap{\gets_+}$ & $ik \cdot k$  \\
            trace                       &       & $\mathclap{\gets_+}$ & $ii$          \\
            \bottomrule
        \end{tabular}
    \end{footnotesize}
    \caption{Common matrix operations expressed as \texttt{mapReduce}}\vspace{-2ex}
    \label{tab:mapReduce}
    \vspace{-5ex}
\end{wraptable}


==> fig/opt.tex <==
\tikzstyle{n} = [fill=ACMOrange,    draw=ACMRed,      rectangle, rounded corners, text centered,minimum width=.5cm,minimum height=.5cm]
\tikzstyle{c} = [fill=ACMLightBlue, draw=ACMDarkBlue, cloud, cloud puffs=12, cloud puff arc=110, aspect=1.5, minimum width=1cm, minimum height=1cm]
\tikzstyle{d} = [fill=ACMLightBlue, draw=ACMDarkBlue, cloud, cloud puffs=14, cloud puff arc=180, aspect=1.5, minimum width=1cm, minimum height=1cm]

\begin{figure}[t]
    \centering
    \begin{subcaptionblock}{.33\textwidth}
        \centering
        \begin{tikzpicture}[node distance=.5cm]
            \node[n] (A)                    {\lstinline|a|};
            \node[c] (c) [above=of A]       {};
            \node[n] (B) [above  left=of c] {\lstinline|b|};
            \node[n] (C) [above right=of c] {\lstinline|c|};

            \draw [-latex] (A) to (c);
            \draw [-latex] (c) to (B);
            \draw [-latex] (c) to (C);
        \end{tikzpicture}
        \begin{lstlisting}[basicstyle=\ttfamily\tiny,xleftmargin=1ex,xrightmargin=1ex]
            con c()                 = /*...*/;
            con b(f: Cn[], i: I32) = /*...*/;

            con a()                 = b(c, x);
        \end{lstlisting}
        \caption{Initial Program\label{fig:opt:a}}
    \end{subcaptionblock}%
    \begin{subcaptionblock}{.33\textwidth}
        \centering
        \begin{tikzpicture}[node distance=.5cm]
            \node[n] (A)                    {\lstinline|a|};
            \node[c] (c) [above=of A]       {};
            \node[n] (B) [above  left=of c] {\lstinline|b|};
            \node[n] (C) [above right=of c] {\lstinline|c|};

            \node[d] (d)  [right=of c]       {};
            \node[n] (Bp) [above right=of d] {\lstinline|B|};

            \draw [-latex] (c) to (B);
            \draw [-latex] (c) to (C);

            \draw [-latex] (A) to (d);
            \draw [-latex] (d) to (C);
            \draw [-latex] (d) to (Bp);
            \draw [-latex,dashed] (B) to[bend left] (Bp);
        \end{tikzpicture}
        \begin{lstlisting}[basicstyle=\ttfamily\tiny,xleftmargin=1ex,xrightmargin=1ex]
            con c()                 = /*...*/;
            con b(f: Cn[], i: I32) = /*...*/;
            con B(f: Cn[])         = /*...*/;
            con a()                 = B c;
        \end{lstlisting}
        \caption{Optimistic Transformation\label{fig:opt:b}}
    \end{subcaptionblock}%
    \begin{subcaptionblock}{.33\textwidth}
        \centering
        \begin{tikzpicture}[node distance=.5cm]
            \node[n] (A)                    {\lstinline|a|};
            \node[c] (c) [above=of A]       {};
            \node[n] (B) [above  left=of c] {\lstinline|b|};
            \node[n] (C) [above right=of c] {\lstinline|c|};

            \node[d] (d)  [right=of c]       {};
            \node[n] (Bp) [above right=of d] {\lstinline|B|};

            \draw [-latex] (A) to (c);
            \draw [-latex] (c) to (B);
            \draw [-latex] (c) to (C);

            \draw [-latex] (d) to (C);
            \draw [-latex] (d) to (Bp);
            \draw [-latex,dashed] (B) to[bend left] (Bp);
        \end{tikzpicture}
        \begin{lstlisting}[basicstyle=\ttfamily\tiny,xleftmargin=1ex,xrightmargin=1ex]
            con c()                 = /*...*/;
            con b(f: Cn[], i: I32) = /*...*/;
            con B(f: Cn[])         = /*...*/;
            con a()                 = b(c, x);
        \end{lstlisting}
        \caption{Backtracking\label{fig:opt:c}}
    \end{subcaptionblock}
    \caption{Backtracking in \mimir's Optimizer}\label{fig:opt}
\end{figure}


==> fig/regex_mim.tex <==
% // import plugins that this plugin depends on
% import core;
% import mem;
% import compile;
% plugin direct;

\begin{lstlisting}[label=lst:regex-dialect,caption=RegEx plugin declaration file \enquote{\texttt{regex.mim}},float=tp]
    // locals
    let Char = I8;
    lam Str(n: Nat): * = %mem.Ptr <<n; Char>>;
    lam Res(n: Nat): * = [%mem.M, Bool, Idx n];
    let RE = PI[n: Nat][%mem.M, Str n, Idx n] -> Res n;

    // regex plugin axioms
    axm %regex.conj:  PI.[n: Nat][<<n; RE>>] -> RE, normalize_conj, 2;
    axm %regex.disj:  PI.[n: Nat][<<n; RE>>] -> RE, normalize_disj, 2;
    axm %regex.range: <<2; Char>> -> RE, normalize_range, 1;
    axm %regex.not_:  RE -> RE, normalize_not, 1;
    axm %regex.any:   RE, normalize_any, 0;
    axm %regex.quant(optional,star,plus): RE -> RE, normalize_quant, 1;

    // regex plugin annexes
    lam %regex.lit (val: Char) = %regex.range (val, val);
    let %regex.cls.w = %regex.disj (%regex.range ('0', '9'), %regex.range ('a', 'z'),
                            %regex.range ('A', 'Z'), %regex.lit '_');
    let %regex.cls.W = %regex.not_ %regex.cls.w; // ditto: %regex.cls.d,D,s,S, ...

    axm %regex.lower_regex: %compile.Pass; // declare the pass of this plugin

    // implementation of matchers
    fun %regex.match_range(l u: Char)(n: Nat)(mem: %mem.M, str: Str n, pos: Idx n): Res n =
      let ptr          = %mem.lea (str, pos);         // get address of current char,
      let (`mem, char) = %mem.load (mem, ptr);        // load, and check range:
      let in_range     = %core.bit2.and_ 0 (%core.icmp.uge (char, l), %core.icmp.ule (char, u));
      let `pos         = (pos, /*pos + 1*/)#in_range; // pos = in_range ? pos : pos + 1
      return (mem, in_range, pos);                     // invoke return continuation
    // %regex.match_not, match_any, match_conj, ...
\end{lstlisting}


==> fig/rewrite.tex <==
\begin{lstlisting}[language=C++,literate=,morekeywords={size_t},float=t,caption=C++ implementation that recursively rewrites a \mimir program (slightly simplified),label=lst:rewrite]
    const Def* rewrite(Def2Def& old2new, const Def* old_def) {
        if (old2newcontains(old_def)) return old2new[old_def];

        size_t n = old_def->num_ops();
        const Def* new_type = rewrite(old2new, old_def->type());

        if (Def* old_mut = old_def->isa_mut()) { // if old_def is a mutable, remove "const"
            Def* new_mut = old_mut->stub(new_type);
            old2new[old_mut] = new_mut; // mutables may be recursive: first put stub into map
            for (size_t i = 0; i != n; ++i) new_mut->set(i, rewrite(old2new, old_mut->op(i)));
            return new_mut;
        }
        // old_def is an immutable
        DefArray new_ops(n); // array with n elements
        for (size_t i = 0; i != n; ++i) new_ops[i] = rewrite(old2new, old_def->op(i));
        const Def* new_def = old_def->rebuild(new_type, new_ops);
        return old2new[old_def] = new_def;
    }
\end{lstlisting}



==> fig/sea_of_nodes.tex <==
\tikzstyle{n} = [fill=ACMOrange,    draw=ACMRed,      rectangle, rounded corners, text centered,minimum width=.5cm,minimum height=.5cm]
\tikzstyle{c} = [fill=ACMLightBlue, draw=ACMDarkBlue, cloud, cloud puffs=12, cloud puff arc=110, aspect=1.5, minimum width=1cm, minimum height=1cm]
\tikzstyle{d} = [fill=ACMLightBlue, draw=ACMDarkBlue, cloud, cloud puffs=14, cloud puff arc=180, aspect=1.5, minimum width=1cm, minimum height=1cm]

\contourlength{1.5pt}
\contournumber{25}
\begin{figure}[t]
    \centering
    \begin{subcaptionblock}{\textwidth}
        \centering
        \begin{tikzpicture}
            \node[] (Lam)      at (0,0) {Lam};
            \node[] (name)     at (-2,-1) {"f"};
            \node[] (arg)      at (0,-1) {:};
            \node[] (arg_name) at (-0.5,-2) {"a"};
            \node[] (I32)      at (1.5,-2) {I32};
            \node[] (app)      at (3.5,-1) {App};
            \node[] (add)      at (2.5,-2) {add};
            \node[] (add_arg)  at (4,-2) {()};
            \node[] (lit)      at (4.5,-3) {Lit};
            \node[] (42)       at (4.5,-4) {42};

            % below others
            \path [->] (add_arg) edge (arg);
            
            \path [->] (Lam) edge node {\tiny\contour{white}{Name}} (name);
            \path [->] (Lam) edge node [pos=0.30] {\tiny\contour{white}{Return}} (I32);
            \path [->] (Lam) edge node {\tiny\contour{white}{Arg}} (arg);
            \path [->] (Lam) edge node {\tiny\contour{white}{Body}} (app);
            
            \path [->] (arg) edge (arg_name);
            \path [->] (arg) edge (I32);
            
            \path [->] (app) edge (add);
            \path [->] (app) edge (add_arg);
            
            \path [->] (add_arg) edge (lit);
            \path [->] (lit) edge (42);
            \path [->] (lit) edge (I32);
        \end{tikzpicture}
        \begin{lstlisting}[basicstyle=\ttfamily\tiny,xleftmargin=1ex,xrightmargin=1ex]
            lam f(a:I32) = add (a, 42:I32);
        \end{lstlisting}
        % \caption{\label{fig:opt:c}}
    \end{subcaptionblock}
    \caption{\mimir's graph based program representation}\label{fig:sea_of_nodes}
\end{figure}


==> fig/tensor.tex <==
\begin{lstlisting}[float=t,caption={The \texttt{\%tensor} plugin (excerpt). Normalizer information has been elided.},label=lst:tensor]
axm %tensor.zip:
    PI.[r: Nat, s: <<r; Nat>>, ni: Nat, Is: <<ni; *>>, no: Nat, Os: <<no; *>>]
      [f: <<i: ni; Is#i>> -> <<o: no; Os#o>>]
      [is: <<i: ni; <<s; Is#i>>>>] -> <<o: no; <<s; Os#o>>>>;
axm %tensor.map:
    PI.[r: Nat, s: <<r; Nat>>, ni: Nat, Is: <<ni; *>>, O: *]
      [f: <<i: ni; Is#i>> -> O]
      [is: <<i: ni; <<s; Is#i>>>>, dims: <<r; Bool>>] -> <<s; O>>;
axm %tensor.reduce:
    PI.[r: Nat, s: <<r; Nat>>, ni: Nat, Is: <<ni; *>>]
      [f: <<2; <<i: ni; Is#i>>>> -> <<i: ni; Is#i>>]
      [is: <<i: ni; <<s; Is#i>>>>, init: <<i: ni; Is#i>>, dims: <<r; Bool>>]
    -> <<i: ni; <<<j: r; (s#j, 1)#(dims#j)>; Is#i>>>>;
\end{lstlisting}


==> fig/time_crop.tex <==
\begin{footnotesize}
\addtolength{\tabcolsep}{-4pt}
\begin{tabular}{l*{6}{c}} \toprule
                                 % & \mimir & \mimir + \clang \verb|O3| & \haskell \verb|O3| & \ocaml \verb|O3| & \rust \verb|Release| & \rust \verb|Static| \\ \midrule
                                 & \mimir & \mimir$^\star$ & \haskell & \ocaml & \rust & \rust \verb|S| \\ \midrule
    \verb|PreOpt|                & \gradient{360} & \gradient{268} & \gradient{403} & \gradient{843} &  &  \\
    \verb|Optimized|             & \gradient{144} & \gradient{138} & \gradient{239} & \gradient{306} &  &  \\
    \verb|Manual|                & \gradient{145} & \gradient{148} & \gradient{153} & \gradient{710} & \gradient{785} & \gradient{179} \\
    \verb|PE (Manual)|  & \gradient{155} & \gradient{148} & \gradient{199} & \gradient{ 80} & \gradient{117} & \gradient{100} \\
    \verb|FE (Manual|)     & \gradient{ 17} & \gradient{  1} & \gradient{ 22} & \gradient{ 24} & \gradient{  1} & \gradient{  1} \\ \bottomrule
\end{tabular}
\addtolength{\tabcolsep}{4pt}
% PE = Partial Eval
% FE = Full Eval
% S = Static
\end{footnotesize}


==> fig/time_crop_pgf.tex <==

    \pgfplotsset{
        colormap/RdBu,
    }
\pgfplotstableset{
        /color cells/min/.initial=0,
        /color cells/max/.initial=1000,
        /color cells/textcolor/.initial=,
        %
        % Usage: 'color cells={min=<value which is mapped to lowest color>,
        %   max = <value which is mapped to largest>}
        color cells/.code={%
            \pgfqkeys{/color cells}{#1}%
            \pgfkeysalso{%
                postproc cell content/.code={%
                    %
                    \begingroup
                    %
                    % acquire the value before any number printer changed
                    % it:
                    \pgfkeysgetvalue{/pgfplots/table/@preprocessed cell content}\value
                    \ifx\value\empty
                        \endgroup
                    \else
                    \pgfmathfloatparsenumber{\value}%
                    \pgfmathfloattofixed{\pgfmathresult}%
                    \let\value=\pgfmathresult
                    %
                    % map that value:
                    \pgfplotscolormapaccess
                        [\pgfkeysvalueof{/color cells/min}:\pgfkeysvalueof{/color cells/max}]
                        {\value}
                        {\pgfkeysvalueof{/pgfplots/colormap name}}%
                    % now, \pgfmathresult contains {<R>,<G>,<B>}
                    %
                    % acquire the value AFTER any preprocessor or
                    % typesetter (like number printer) worked on it:
                    \pgfkeysgetvalue{/pgfplots/table/@cell content}\typesetvalue
                    \pgfkeysgetvalue{/color cells/textcolor}\textcolorvalue
                    %
                    % tex-expansion control
                    % see https://tex.stackexchange.com/questions/12668/where-do-i-start-latex-programming/27589#27589
                    \toks0=\expandafter{\typesetvalue}%
                    \xdef\temp{%
                        \noexpand\pgfkeysalso{%
                            @cell content={%
                                \noexpand\cellcolor[rgb]{\pgfmathresult}%
                                \noexpand\definecolor{mapped color}{rgb}{\pgfmathresult}%
                                \ifx\textcolorvalue\empty
                                \else
                                    \noexpand\color{\textcolorvalue}%
                                \fi
                                \the\toks0 %
                            }%
                        }%
                    }%
                    \endgroup
                    \temp
                    \fi
                }%
            }%
        }
    }

    \pgfplotstabletypeset[
        color cells={
            % provide suitable `min' and `max' values.
            % The mean value of these will show as white
            min=0,
            max=100,
        },
        col sep=comma,
    ]{
        0,55,100,0,0,0,7,16,10,19,21,29
        43,43,90,17,87,8,20,81,43,20,18,31
        67,21,50,0,70,5,6,5,26,23,20,25
        11,40,60,63,7,14,10,17,24,22,15,38
        25,0,33,50,17,16,9,10,22,6,19,22
        22,5,0,0,2,50,0,3,8,7,13,18
        0,50,30,40,50,1,20,13,3,12,5,11
    }

